SLD-Resolution Reduction of Second-Order Horn Fragments -- technical report --

We present the derivation reduction problem for SLD-resolution, the undecidable problem of finding a finite subset of a set of clauses from which the whole set can be derived using SLD-resolution. We study the reducibility of various fragments of second-order Horn logic with particular applications in Inductive Logic Programming. We also discuss how these results extend to standard resolution.

==> 01-decidability_results.tex <==

We now show that the reduction$_\res$ and reduction$_\sld$ problems are both undecidable. We also show how these problems relate to one another. We first reiterate the subsumption theorem for resolution, which uses the notion of a deduction \cite{ilp:book}:

\begin{definition}[Resolution deduction]
Let $T$ be a clausal theory and $C$ be a clause. Then there exists a deduction of $C$ from $T$, written $T \vdash_d C$, if $C$ is a tautology or if there exists a clause $D$ such that $T \vdash_d D$ and $D$ subsumes $C$.
\end{definition}

We can now restate the subsumption theorem for resolution \cite{ilp:book}:

\begin{theorem}[Subsumption theorem for resolution]
Let $T$ be a clausal theory and $C$ be a Clause. Then $T \models C$ if and only if $T \vdash_d C$.
\end{theorem}

We can now show that the reduction$_\res$ problem is undecidable:
\begin{theorem}[Reduction$_\res$ undecidability]
  \label{prop-clausal-undecidability}
  The reduction$_\res$ problem is undecidable.
\end{theorem}
\begin{proof}
  Assume the problem is decidable, which implies that $T \vdash_\res^* C$ is decidable. Since $T \vdash_\res^* C$ is decidable and subsumption between clauses is decidable \cite{DBLP:books/fm/GareyJ79}, then finding a deduction is decidable. Therefore, by the subsumption theorem for resolution, entailment between clauses is decidable. However, entailment between clauses is undecidable \cite{schmid-schauss}, so the assumption cannot hold. Therefore, the problem must be undecidable.
\end{proof}

We can use the same reasoning to show that the reduction$_\sld$ problems is also undecidable:
\begin{theorem}[Reduction$_\sld$ undecidability]
  The reduction$_\sld$ problem for Horn theories is undecidable.
\end{theorem}
\begin{proof}
  Follows using the same argument as in Th.\ \ref{prop-clausal-undecidability}
  based on the subsumption theorem for SLD-resolution \cite{ilp:book} and using
  the undecidability of entailment between Horn clauses \cite{horn:undecidable}.
\end{proof}

Both problems are undecidable and they relate to each other as described in Th.\ \ref{th:stor}.
The proof of this theorem relies on the following simple result:

\begin{proposition}
  \label{prop:finite}
  Any theory that is finite has a minimal$_\gen$ core.
\end{proposition}
\begin{theorem}[Relation between reduction$_\sld$ and reduction$_\res$]
  \label{th:stor}
  If a theory $T$ has a minimal$_\sld$ core $T'$ then it also admits a minimal$_\res$ core included in $T'$.
\end{theorem}
\begin{proof}
  SLD-resolution is a restriction of resolution, thus any derivation by the former is also a derivation by the latter.
  Hence $T'\vdash_\sld^* T$ implies $T'\vdash_\res^* T$.
  Moreover $T'$ is finite, thus by Prop.\ \ref{prop:finite} it has a minimal$_\res$ core $T''$.
  By definition, $T''$ is reduced$_\res$, and $T''\vdash_\res^*T'\vdash_\res^*T$, thus $T''$ is a minimal$_\res$ core of $T$.
\end{proof}


==> 02-reducible_fragments.tex <==
\begin{proposition}[Reducible fragment]
  \label{prop:freduc}
  If a fragment \F\ of \Horn\ is reducible$_\gen$ to $\F_{\infty,b}$ then \F\ is redundant$_\gen$ to $\F_{\infty,b}$.
\end{proposition}
\begin{proof}
  We show the property by induction on the body size of the clauses.
  Let us consider $C\in\F$ such that $\bsize{C}=b+1$.
  Due to the reducibility$_\gen$ of \F\ to $\F_{\infty,b}$, $C$ can be generated by $C_1$ and $C_2$ such that $\bsize{C_1}\leq b$ and $\bsize{C_2}\leq b$, hence the property is verified.

  Now we assume that the property is verified for any clause of body size smaller or equal to a given $b'\geq b+1$.
  Let us consider the clause $C\in\F$ such that $\bsize{C}=b'+1$.
  Since \F\ is reducible$_\gen$ to $\F_{\infty,b}$, there exist $C_1,C_2\in\F_{\infty,b'}$ such that $C_1,C_2\vdash_\gen C$.
  By induction, $\F_{\infty,b}\vdash_\gen^* C_1$ and $\F_{\infty,b}\vdash_\gen^* C_2$.
  Hence $\F_{\infty,b}\vdash_\gen^* C$.
\end{proof}
\begin{theorem}[Cores of reducible fragments]
  If a fragment \F\ is reducible to $\F_{\infty,b}$ then the solutions of the reduction$_\gen$ problem for \F\ and $\F_{\infty,b}$ coincide, i.e.\ if there are any, the minimal$_\gen$ cores of \F\ coincide.
\end{theorem}
\begin{proof}
  Let \F\ be a fragment of \Horn\ reducible$_\gen$ to $\F_{\infty,b}$.
  First, we assume that $\F_{\infty,b}$ has a minimal$_\gen$ core $\F'$.
  Then $\F_{\infty,b}$ is redundant$_\gen$ to $\F'$ and by Prop.\ \ref{prop:freduc} \F\ is redundant$_\gen$ to $\F_{\infty,b}$ thus point (1) of the reduction problem is satisfied.
  Moreover, $\F'$ also satisfies point (2) due to being a minimal$_\gen$ core of $\F_{\infty,b}$, thus $\F'$ is also a minimal$_\gen$ core of \F.
  Now we assume that $\F'$ is a minimal$_\gen$ core of \F.
  Since $\F_{\infty,b}\subseteq\F$ and $\F'\vdash_\gen^*\F$, it is also true that $\F'\vdash_\gen^*\F_{\infty,b}$, satisfying point (1) of the reduction problem for $\F_{\infty,b}$.
  In addition, $\F'$ is reduced$_\gen$, i.e.\ point (2) is also satisfied.
  Hence $\F'$ is also a minimal$_\gen$ core of $\F_{\infty,b}$.
\end{proof}



==> 04-cbase.tex <==
\begin{proposition}[Non-reducibility$_\sld$ of \cbase]
  \label{prop:base}
  $\cbase$ is not reducible$_\sld$.
\end{proposition}
\begin{proof}
  To derive$_\sld$ the clause \cbase\ from two smaller clauses, these two smaller clauses $C_1$ and $C_2$ must form a partition of the literals in \cbase\ if one excludes the pivot.
  Let us consider the possible partitions of \cbase.
  Each of the two sets in the partition must contain at least two elements, otherwise one of $C_1$, $C_2$ would be as big as \cbase, which we want to avoid.
  There are a total of 6 literals in \cbase\, thus the only partitions of interest are the ones with a 2-4 ratio and a 3-3 ratio, for a total of 25 cases (15 2-4 cases and half of the 20 3-3 cases since we do not care which clause gets which set of literals).
  Due to the symmetries of the problem, a great number of cases can be safely skipped, reducing the number of cases to consider to only 4.
  \begin{enumerate}
  \item Assume $P_0(x_1,x_2)$ and $P_1(x_1,x_3)$ are the only literals of \cbase\ that belong to $C_1$.
    Then, for $C_1$ and $C_2$ to both be in \chainmost{2}, the pivot needs to contain at least the variables $x_1$ (pending in $C_2$) and $x_2$, $x_3$ (pending in $C_1$).
    Since these clauses contain at most dyadic literals, this is not possible.
    All the 2-4 cases where there is one term variable that connects the two literals occurring in the smaller subset of size two, in either $C_1$ or $C_2$, are symmetrical to this one and thus also impossible to fulfill.
  \item Assume $P_0(x_1,x_2)$ and $P_5(x_3,x_4)$ are the only literals of \cbase\ that belong to $C_1$.
    Then, the resolving literal needs to contain all the four variables for $C_1$ and $C_2$ to belong to \chainmost{2}, which is not possible.
    All the remaining 2-4 cases are symmetrical to this one.
  \item Assume $P_0(x_1,x_2)$, $P_1(x_1,x_3)$ and $P_2(x_1,x_4)$ are the only literals of \cbase\ in $C_1$.
    Then, $x_2$, $x_3$ and $x_4$ must occur in the resolving literal, which is impossible.
    All the 3-3 cases where the three literals share a common variable are symmetrical.
  \item Assume $P_1(x_1,x_2)$, $P_2(x_1,x_4)$ and $P_3(x_2,x_3)$ are the only literals of \cbase\ in $C_1$.
    Then, all four variables must occur in the resolving literal, which is impossible.
    All the remaining 3-3 cases are symmetrical to this one.
  \end{enumerate}
  Thus it is not possible to reduce$_{\sld}$ \cbase.
\end{proof}


